Understanding the Impact of Culture in Assessing Helpfulness of Online Reviews

Online reviews have become essential for users to make informed decisions in everyday tasks ranging from planning summer vacations to purchasing groceries and making financial investments. A key problem in using online reviews is the overabundance of online that overwhelms the users. As a result, recommendation systems for providing helpfulness of reviews are being developed. This paper argues that cultural background is an important feature that impacts the nature of a review written by the user, and must be considered as a feature in assessing the helpfulness of online reviews. The paper provides an in-depth study of differences in online reviews written by users from different cultural backgrounds and how incorporating culture as a feature can lead to better review helpfulness recommendations. In particular, we analyze online reviews originating from two distinct cultural spheres, namely Arabic and Western cultures, for two different products, hotels and books. Our analysis demonstrates that the nature of reviews written by users differs based on their cultural backgrounds and that this difference varies based on the specific product being reviewed. Finally, we have developed six different review helpfulness recommendation models that demonstrate that taking culture into account leads to better recommendations.

==> aspect-analysis.tex <==
\subsection{Review Aspects Analysis}
\label{subsec:aspects-analysis}
We now turn into studying the correlation between product aspects and culture to understand if different cultures are concerned with different aspects of the product. Our analysis inspected aspects studied in aspect analysis research for hotels \cite{akhtar2017aspect} and books \cite{al2015human} where we looked at the 10 hotel aspects and 7 book aspects shown in Figures \ref{fig:aspects-hotels} and \ref{fig:aspects-books} respectively. We used the appearance of the aspect in the text review as an indicator for the interest of reviewers in this aspect. It is important to note that an aspect can be discussed by mentioning sub-aspects under the main aspect and sub-aspects can also have synonyms in both languages. Hence, we compiled a list of words corresponding to each aspect for each language as shown in Table \ref{table:hotel-aspects}. To extract these sub-aspects and their synonyms, we counted the most frequent 100 words in each dataset. After that, we manually inspected the meaning of these words to see whether each word fits under an aspect category. This work has been done by the authors of this paper as they are capable of speaking both English and Arabic.

\begin{table}
\caption{ADD CAPTION HERE}
\label{table:hotel-aspects}
\centering
\begin{tabular}{|c|c|c|} 
 \hline
 Aspect & English & Arabic \\ 
 \hline
 Food & cell5 &  cell9 \\ 
 \hline
 Location & cell8 & cell9 \\ 
 \hline
 Service & cell8 & cell9 \\ 
 \hline
 Staff & cell8 & cell9 \\ 
 \hline
 Bed & cell8 & cell9 \\ 
 \hline
 Bathroom & cell8 & cell9 \\ 
 \hline
 Internet & cell8 & cell9 \\ 
 \hline
 Cleanliness & cell8 & cell9 \\ 
 \hline
 Parking & cell8 & cell9 \\ 
 \hline
 Price & cell8 & cell9 \\
 \hline

\end{tabular}

\end{table}

Figures \ref{fig:aspects-hotels} and \ref{fig:aspects-books} plot the percentage of reviews discussing a particular aspect by at least mentioning one of its corresponding words from Table \ref{Table:xxx}. Note that it is normal to encounter a review discussing more than one aspect. We see from Figure \ref{fig:aspects-hotels} that location, staff and food are the top discussed aspects for both cultures with English reviewers discussing aspects more than Arabic reviewers in the three cases. We also note that the price, cleanliness and food are discussed almost equally for both cultures hence having almost similar importance. A clear difference can be seen in the aspects of service, bed, bathroom, Internet and parking. For these five cases, Arabic reviewers are more concerned with the service, quality of the parking  and the Internet whereas English reviewers value aspects related to the bed and the bathroom more. We now turn into discussing book aspects as seen in Figure \ref{fig:aspects-books}. Again, the top 3 discussed aspects are similar for both cultures being the style, plot and feelings. However, English reviewers have the style as their top discussed aspect being mentioned in 77\% of the reviews whereas for Arabic reviewers the feelings and the plot are the most discussed having been discussed in 51\% of the reviews for both aspects. The great difference appears in the character aspect being discussed in 39\% of the English reviews compared to only 18\% in Arabic reviews. An important observation that follows from observing all aspects is that English reviewers focus more on mentioning the aspects of the book compared to Arabic reviews who also discuss aspects but at lesser extent or percentages.

\begin{figure*}
\centering
\includegraphics[scale=0.5, width=12cm]{img/Aspects-Books.pdf}

\caption{INCLUDE CAPTION HERE}
\label{fig:aspects-hotels}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[scale=0.5, width=12cm]{img/Aspects-Hotels.pdf}
\caption{INCLUDE CAPTION HERE}
\label{fig:aspects-books}
\end{figure*}


